SafeFlowMPC: Predictive and Safe Trajectory Planning for Robot Manipulators with Learning-based Policies

The emerging integration of robots into everyday life brings several major challenges. Compared to classical industrial applications, more flexibility is needed in combination with real-time reactivity. Learning-based methods can train powerful policies based on demonstrated trajectories, such that the robot generalizes a task to similar situations. However, these black-box models lack interpretability and rigorous safety guarantees. Optimization-based methods provide these guarantees but lack the required flexibility and generalization capabilities. This work proposes SafeFlowMPC, a combination of flow matching and online optimization to combine the strengths of learning and optimization. This method guarantees safety at all times and is designed to meet the demands of real-time execution by using a suboptimal model-predictive control formulation. SafeFlowMPC achieves strong performance in three real-world experiments on a KUKA 7-DoF manipulator, namely two grasping experiment and a dynamic human-robot object handover experiment. A video of the experiments is available at http://www.acin.tuwien.ac.at/42d6. The code is available at https://github.com/TU-Wien-ACIN-CDS/SafeFlowMPC.

==> data/scen_global_planner.tex <==
\begin{tikzpicture}
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{acinblue}{RGB}{0,102,153}
	\definecolor{acinyellow}{RGB}{252, 204, 71}
	\definecolor{acingreen}{RGB}{0,190,65}
	\definecolor{acinred}{RGB}{186,18,43}
	\definecolor{lightgray204}{RGB}{204,204,204}

	% \node[inner sep=0pt, opacity=0.5] (qf) at (4.05,1.8)
	% {\includegraphics[width=.185\textwidth]{data/scen0_qf_t.png}};
	% \node[inner sep=0pt, opacity=0.5] (q0) at (4.05,1.8)
	% {\includegraphics[width=.185\textwidth]{data/scen0_q0_t.png}};
	% \node[inner sep=0pt, opacity=0.5] (q0) at (3.75,1.90)
	% {\includegraphics[width=.13\textwidth]{inkscape/robots_scen0.eps}};
	%
	\begin{axis}[
			view={60}{11},
			xlabel={$x$ / \si{\meter}},
			ylabel={$y$ / \si{\meter}},
			zlabel={$z$ / \si{\meter}},
			zmin=0,
			xmin=-1,
			xmax=1,
			axis equal,
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			y grid style={darkgray176},
			xtick style={color=black},
			ytick style={color=black},
			legend cell align={left},
			legend style={
					fill opacity=0.8,
					draw opacity=1,
					text opacity=1,
					draw=lightgray204,
				},
			legend entries ={SafeFlowMPC, BoundPlanner, VP-STO}
		]
		\pgfplotstableread{data/p_BoundMPC.txt}\pbmpc;
		\pgfplotstableread{data/r_BoundMPC.txt}\rbmpc;
		\pgfplotstableread{data/p_SafeFlowMPC.txt}\psfmpc;
		\pgfplotstableread{data/r_SafeFlowMPC.txt}\rsfmpc;
		\pgfplotstableread{data/p_VPSTO.txt}\pgp;
		\pgfplotstableread{data/r_VPSTO.txt}\rgp;
		%
		% \addplot3 [black, thick]
		% table [
		% 		x expr=\thisrowno{0},
		% 		y expr=\thisrowno{1},
		% 		z expr=\thisrowno{2}
		% 	] {\ptraj};
		%
		% \addplot3 [acinred, thick]
		% table [
		% 		x expr=\thisrowno{0},
		% 		y expr=\thisrowno{1},
		% 		z expr=\thisrowno{2}
		% 	] {\pgcs};
		%
		% \addplot3 [acinblue, thick]
		% table [
		% 		x expr=\thisrowno{0},
		% 		y expr=\thisrowno{1},
		% 		z expr=\thisrowno{2}
		% 	] {\ptracking};
		%
		% \addplot3 [acingreen, thick]
		% table [
		% 		x expr=\thisrowno{0},
		% 		y expr=\thisrowno{1},
		% 		z expr=\thisrowno{2}
		% 	] {\pvpsto};


		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acinred] coordinates
			{
				(1.1,0.05,0.7300000000000001) (0.55,-0.05,0.7300000000000001) (1.1,-0.05,0.7300000000000001)
				(1.1,0.05,0.7300000000000001) (0.55,-0.05,0.7300000000000001) (0.55,0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001) (0.55,0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (0.55,-0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (0.55,0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (1.1,0.05,0.8699999999999999)
				(1.1,-0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001) (1.1,-0.05,0.7300000000000001)
				(1.1,-0.05,0.8699999999999999) (0.55,-0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001)
				(1.1,-0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (1.1,-0.05,0.7300000000000001)
				(1.1,-0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (1.1,0.05,0.8699999999999999)
				(1.1,-0.05,0.8699999999999999) (0.55,0.05,0.8699999999999999) (0.55,-0.05,0.8699999999999999)
				(1.1,-0.05,0.8699999999999999) (0.55,0.05,0.8699999999999999) (1.1,0.05,0.8699999999999999)
			};
		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acinred] coordinates
			{
				(1.1,0.05,0.0) (0.55,-0.05,0.0) (1.1,-0.05,0.0)
				(1.1,0.05,0.0) (0.55,-0.05,0.0) (0.55,0.05,0.0)
				(0.55,0.05,0.35) (0.55,-0.05,0.0) (0.55,0.05,0.0)
				(0.55,0.05,0.35) (0.55,-0.05,0.35) (0.55,-0.05,0.0)
				(0.55,0.05,0.35) (1.1,0.05,0.0) (0.55,0.05,0.0)
				(0.55,0.05,0.35) (1.1,0.05,0.0) (1.1,0.05,0.35)
				(1.1,-0.05,0.35) (0.55,-0.05,0.0) (1.1,-0.05,0.0)
				(1.1,-0.05,0.35) (0.55,-0.05,0.35) (0.55,-0.05,0.0)
				(1.1,-0.05,0.35) (1.1,0.05,0.0) (1.1,-0.05,0.0)
				(1.1,-0.05,0.35) (1.1,0.05,0.0) (1.1,0.05,0.35)
				(1.1,-0.05,0.35) (0.55,0.05,0.35) (0.55,-0.05,0.35)
				(1.1,-0.05,0.35) (0.55,0.05,0.35) (1.1,0.05,0.35)
			};
		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acinred] coordinates
			{
				(0.48055403773216077,-0.4861009349781342,0.14000100946302307) (0.6793232814623744,-0.4639472051160296,0.1400013497625498) (0.6737848489969847,-0.41425489418345435,0.1400
				0126873896454)
				(0.48055403773216077,-0.4861009349781342,0.14000100946302307) (0.6737848489969847,-0.41425489418345435,0.14000126873896454) (0.475015605266771,-0.43640862404555897,0.140
				00092843943782)
				(0.6737850360494299,-0.4142550363861625,0.04000126873924057) (0.6793232814623744,-0.4639472051160296,0.1400013497625498) (0.6737848489969847,-0.41425489418345435,0.14000
				126873896454)
				(0.6737850360494299,-0.4142550363861625,0.04000126873924057) (0.6793232814623744,-0.4639472051160296,0.1400013497625498) (0.6793234685148195,-0.4639473473187377,0.040001
				34976282585)
				(0.4750157923192162,-0.43640876624826713,0.040000928439713826) (0.6737848489969847,-0.41425489418345435,0.14000126873896454) (0.475015605266771,-0.43640862404555897,0.14
				000092843943782)
				(0.4750157923192162,-0.43640876624826713,0.040000928439713826) (0.6737850360494299,-0.4142550363861625,0.04000126873924057) (0.6737848489969847,-0.41425489418345435,0.14
				000126873896454)
				(0.480554224784606,-0.48610107718084233,0.04000100946329911) (0.48055403773216077,-0.4861009349781342,0.14000100946302307) (0.6793232814623744,-0.4639472051160296,0.1400
				013497625498)
				(0.480554224784606,-0.48610107718084233,0.04000100946329911) (0.6793232814623744,-0.4639472051160296,0.1400013497625498) (0.6793234685148195,-0.4639473473187377,0.040001
				34976282585)
				(0.480554224784606,-0.48610107718084233,0.04000100946329911) (0.6737850360494299,-0.4142550363861625,0.04000126873924057) (0.6793234685148195,-0.4639473473187377,0.04000
				134976282585)
				(0.480554224784606,-0.48610107718084233,0.04000100946329911) (0.4750157923192162,-0.43640876624826713,0.040000928439713826) (0.6737850360494299,-0.4142550363861625,0.040
				00126873924057)
				(0.480554224784606,-0.48610107718084233,0.04000100946329911) (0.48055403773216077,-0.4861009349781342,0.14000100946302307) (0.475015605266771,-0.43640862404555897,0.1400
				0092843943782)
				(0.480554224784606,-0.48610107718084233,0.04000100946329911) (0.4750157923192162,-0.43640876624826713,0.040000928439713826) (0.475015605266771,-0.43640862404555897,0.140
				00092843943782)
			};
		% \addplot3[
		% 	only marks,
		% 	mark=*,
		% 	mark size=1pt,
		% ] coordinates {(0, 0, 0)};
		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates {(0.57716954, -0.45017799, 0.09000114)};
		\draw (axis cs:0.57716954, -0.45017799, 0.09000114) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{f}$};
		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates {(0.34743431, 0.45745164, 0.22161833)};
		\draw (axis cs:0.34743431, 0.45745164, 0.22161833) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_{0}$};

	\end{axis}
\end{tikzpicture}


==> tikz/scen_global_planner.tex <==
\begin{tikzpicture}
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{acinblue}{RGB}{0,102,153}
	\definecolor{acinyellow}{RGB}{252, 204, 71}
	\definecolor{acingreen}{RGB}{0,190,65}
	\definecolor{acinred}{RGB}{186,18,43}
	\definecolor{lightgray204}{RGB}{204,204,204}

	\begin{axis}[
			view={80}{10},
			% in rviz array([0.5       , 0.40557979, 0.5       , 0.57922797])
			xlabel={$x$ / \si{\meter}},
			ylabel={$y$ / \si{\meter}},
			zlabel={$z$ / \si{\meter}},
			zmin=0,
			xmin=-1,
			xmax=1,
			axis equal,
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			y grid style={darkgray176},
			xtick style={color=black},
			ytick style={color=black},
			legend cell align={left},
			legend style={
					fill opacity=0.8,
					draw opacity=1,
					text opacity=1,
					draw=lightgray204,
				},
			legend entries ={SafeFlowMPC, BoundPlanner, VP-STO}
		]

		\node[inner sep=0pt, opacity=0.5] (qf) at (axis cs:0, 0.135, 0.36)
		{\includegraphics[width=.415\textwidth]{tikz/exp1_robot_q0_t.png}};
		\node[inner sep=0pt, opacity=0.5] (qf) at (axis cs:0, 0.135, 0.36)
		{\includegraphics[width=.415\textwidth]{tikz/exp1_robot_q18_t.png}};
		\node[inner sep=0pt, opacity=0.5] (qf) at (axis cs:0, 0.135, 0.36)
		{\includegraphics[width=.415\textwidth]{tikz/exp1_robot_qf_t.png}};


		\pgfplotstableread{data/p_BoundMPC.txt}\pbmpc;
		\pgfplotstableread{data/r_BoundMPC.txt}\rbmpc;
		\pgfplotstableread{data/p_SafeFlowMPC.txt}\psfmpc;
		\pgfplotstableread{data/r_SafeFlowMPC.txt}\rsfmpc;
		\pgfplotstableread{data/p_VPSTO.txt}\pgp;
		\pgfplotstableread{data/r_VPSTO.txt}\rgp;
		%
		\addplot3 [acinred, thick]
		table [
				x expr=\thisrowno{0},
				y expr=\thisrowno{1},
				z expr=\thisrowno{2}
			] {\pgp};
		%
		\addplot3 [acinblue, thick]
		table [
				x expr=\thisrowno{0},
				y expr=\thisrowno{1},
				z expr=\thisrowno{2}
			] {\psfmpc};
		%
		\addplot3 [acinyellow, thick]
		table [
				x expr=\thisrowno{0},
				y expr=\thisrowno{1},
				z expr=\thisrowno{2}
			] {\pbmpc};
		%
		% \addplot3 [acingreen, thick]
		% table [
		% 		x expr=\thisrowno{0},
		% 		y expr=\thisrowno{1},
		% 		z expr=\thisrowno{2}
		% 	] {\pvpsto};


		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acinred] coordinates
			{
				(1.1,0.05,0.7300000000000001) (0.55,-0.05,0.7300000000000001) (1.1,-0.05,0.7300000000000001)
				(1.1,0.05,0.7300000000000001) (0.55,-0.05,0.7300000000000001) (0.55,0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001) (0.55,0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (0.55,-0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (0.55,0.05,0.7300000000000001)
				(0.55,0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (1.1,0.05,0.8699999999999999)
				(1.1,-0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001) (1.1,-0.05,0.7300000000000001)
				(1.1,-0.05,0.8699999999999999) (0.55,-0.05,0.8699999999999999) (0.55,-0.05,0.7300000000000001)
				(1.1,-0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (1.1,-0.05,0.7300000000000001)
				(1.1,-0.05,0.8699999999999999) (1.1,0.05,0.7300000000000001) (1.1,0.05,0.8699999999999999)
				(1.1,-0.05,0.8699999999999999) (0.55,0.05,0.8699999999999999) (0.55,-0.05,0.8699999999999999)
				(1.1,-0.05,0.8699999999999999) (0.55,0.05,0.8699999999999999) (1.1,0.05,0.8699999999999999)
			};
		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acinred] coordinates
			{
				(1.1,0.05,0.0) (0.55,-0.05,0.0) (1.1,-0.05,0.0)
				(1.1,0.05,0.0) (0.55,-0.05,0.0) (0.55,0.05,0.0)
				(0.55,0.05,0.35) (0.55,-0.05,0.0) (0.55,0.05,0.0)
				(0.55,0.05,0.35) (0.55,-0.05,0.35) (0.55,-0.05,0.0)
				(0.55,0.05,0.35) (1.1,0.05,0.0) (0.55,0.05,0.0)
				(0.55,0.05,0.35) (1.1,0.05,0.0) (1.1,0.05,0.35)
				(1.1,-0.05,0.35) (0.55,-0.05,0.0) (1.1,-0.05,0.0)
				(1.1,-0.05,0.35) (0.55,-0.05,0.35) (0.55,-0.05,0.0)
				(1.1,-0.05,0.35) (1.1,0.05,0.0) (1.1,-0.05,0.0)
				(1.1,-0.05,0.35) (1.1,0.05,0.0) (1.1,0.05,0.35)
				(1.1,-0.05,0.35) (0.55,0.05,0.35) (0.55,-0.05,0.35)
				(1.1,-0.05,0.35) (0.55,0.05,0.35) (1.1,0.05,0.35)
			};
		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acingreen] coordinates
			{
				(0.6643815288212902,0.2947798213329385,0.19998135338542958) (0.615362408348182,0.4886830882902628,0.09998810915703432) (0.6643857147508129,0.2947843637361393,0.09998135357620673)
				(0.6643815288212902,0.2947798213329385,0.19998135338542958) (0.615362408348182,0.4886830882902628,0.09998810915703432) (0.6153582224186596,0.48867854588706217,0.19998810896625718)
				(0.6643815288212902,0.2947798213329385,0.19998135338542958) (0.6159068476985213,0.2825239948263581,0.19997876756038113) (0.5668835412958906,0.4764227193804817,0.19998552314120874)
				(0.6643815288212902,0.2947798213329385,0.19998135338542958) (0.6153582224186596,0.48867854588706217,0.19998810896625718) (0.5668835412958906,0.4764227193804817,0.19998552314120874)
				(0.615911033628044,0.28252853722955884,0.09997876775115827) (0.6643815288212902,0.2947798213329385,0.19998135338542958) (0.6159068476985213,0.2825239948263581,0.19997876756038113)
				(0.615911033628044,0.28252853722955884,0.09997876775115827) (0.6643815288212902,0.2947798213329385,0.19998135338542958) (0.6643857147508129,0.2947843637361393,0.09998135357620673)
				(0.5668877272254134,0.4764272617836825,0.09998552333198586) (0.6153582224186596,0.48867854588706217,0.19998810896625718) (0.5668835412958906,0.4764227193804817,0.19998552314120874)
				(0.5668877272254134,0.4764272617836825,0.09998552333198586) (0.615362408348182,0.4886830882902628,0.09998810915703432) (0.6153582224186596,0.48867854588706217,0.19998810896625718)
				(0.5668877272254134,0.4764272617836825,0.09998552333198586) (0.6159068476985213,0.2825239948263581,0.19997876756038113) (0.5668835412958906,0.4764227193804817,0.19998552314120874)
				(0.5668877272254134,0.4764272617836825,0.09998552333198586) (0.615911033628044,0.28252853722955884,0.09997876775115827) (0.6159068476985213,0.2825239948263581,0.19997876756038113)
				(0.5668877272254134,0.4764272617836825,0.09998552333198586) (0.615362408348182,0.4886830882902628,0.09998810915703432) (0.6643857147508129,0.2947843637361393,0.09998135357620673)
				(0.5668877272254134,0.4764272617836825,0.09998552333198586) (0.615911033628044,0.28252853722955884,0.09997876775115827) (0.6643857147508129,0.2947843637361393,0.09998135357620673)
			};
		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates {(0, 0, 0)};
		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates {(0.61563463, 0.38560354, 0.14998344)};
		\draw (axis cs:0.61563463, 0.38560354, 0.14998344) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{f}$};
		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates {(0.45932693, -0.59999839 , 0.4454559 )};
		\draw (axis cs:0.45932693, -0.59999839 , 0.4054559 ) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_{0}$};

	\end{axis}
\end{tikzpicture}


==> tikz/scen_handover.tex <==
\begin{tikzpicture}
	\definecolor{darkgray176}{RGB}{176,176,176}
	\definecolor{acinblue}{RGB}{0,102,153}
	\definecolor{acinyellow}{RGB}{252, 204, 71}
	\definecolor{acingreen}{RGB}{0,190,65}
	\definecolor{acinred}{RGB}{186,18,43}
	\definecolor{lightgray204}{RGB}{204,204,204}

	\begin{axis}[
			view={115}{20},
			% in rviz array([0.30818239, 0.48374946, 0.69086583, 0.44013007])
			xlabel={$x$ / \si{\meter}},
			ylabel={$y$ / \si{\meter}},
			zlabel={$z$ / \si{\meter}},
			zmin=0,
			zmax=1.5,
			xmin=-1,
			xmax=2.5,
			axis equal,
			tick align=outside,
			tick pos=left,
			x grid style={darkgray176},
			y grid style={darkgray176},
			xtick style={color=black},
			ytick style={color=black},
			legend cell align={left},
			legend style={
					fill opacity=0.8,
					draw opacity=1,
					text opacity=1,
					draw=lightgray204,
				},
			legend pos=north east,
			legend entries ={SafeFlowMPC, Human Hand}
		]

		\node[inner sep=0pt, opacity=0.5] (qf) at (axis cs:0.05, 0.03, 0.79)
		{\includegraphics[width=.146\textwidth]{tikz/exp2_robot_q0_t.png}};
		\node[inner sep=0pt, opacity=0.5] (qf) at (axis cs:0.05, 0.03, 0.79)
		{\includegraphics[width=.146\textwidth]{tikz/exp2_robot_qho_t.png}};
		\node[inner sep=0pt, opacity=0.5] (qf) at (axis cs:0.05, 0.03, 0.79)
		{\includegraphics[width=.146\textwidth]{tikz/exp2_robot_qf_t.png}};


		\pgfplotstableread{data/p_SafeFlowMPC_ho.txt}\psfmpc;
		\pgfplotstableread{data/r_SafeFlowMPC_ho.txt}\rsfmpc;
		\pgfplotstableread{data/p_hand.txt}\phand;
		%
		%
		\addplot3 [acinred, thick]
		table [
				x expr=\thisrowno{0},
				y expr=\thisrowno{1},
				z expr=\thisrowno{2}
			] {\psfmpc};
		%
		\addplot3 [acinblue, thick]
		table [
				x expr=\thisrowno{0},
				y expr=\thisrowno{1},
				z expr=\thisrowno{2}
			] {\phand};
		%
		% \addplot3 [acingreen, thick]
		% table [
		% 		x expr=\thisrowno{0},
		% 		y expr=\thisrowno{1},
		% 		z expr=\thisrowno{2}
		% 	] {\pvpsto};

		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acinred] coordinates
			{
				(0.9686957182973392,-0.7330219075336785,0.0) (0.9686957182973394,-1.2330219075336786,2.0) (0.9686957182973392,-0.7330219075336785,2.0)
				(0.9686957182973392,-0.7330219075336785,0.0) (0.9686957182973394,-1.2330219075336786,2.0) (0.9686957182973394,-1.2330219075336786,0.0)
				(0.9686957182973392,-0.7330219075336785,0.0) (0.4686957182973392,-0.7330219075336785,-0.0) (0.4686957182973392,-1.2330219075336784,-0.0)
				(0.9686957182973392,-0.7330219075336785,0.0) (0.9686957182973394,-1.2330219075336786,0.0) (0.4686957182973392,-1.2330219075336784,-0.0)
				(0.4686957182973392,-0.7330219075336785,2.0) (0.9686957182973392,-0.7330219075336785,0.0) (0.4686957182973392,-0.7330219075336785,-0.0)
				(0.4686957182973392,-0.7330219075336785,2.0) (0.9686957182973392,-0.7330219075336785,0.0) (0.9686957182973392,-0.7330219075336785,2.0)
				(0.4686957182973392,-1.2330219075336784,2.0) (0.9686957182973394,-1.2330219075336786,0.0) (0.4686957182973392,-1.2330219075336784,-0.0)
				(0.4686957182973392,-1.2330219075336784,2.0) (0.9686957182973394,-1.2330219075336786,2.0) (0.9686957182973394,-1.2330219075336786,0.0)
				(0.4686957182973392,-1.2330219075336784,2.0) (0.4686957182973392,-0.7330219075336785,-0.0) (0.4686957182973392,-1.2330219075336784,-0.0)
				(0.4686957182973392,-1.2330219075336784,2.0) (0.4686957182973392,-0.7330219075336785,2.0) (0.4686957182973392,-0.7330219075336785,-0.0)
				(0.4686957182973392,-1.2330219075336784,2.0) (0.9686957182973394,-1.2330219075336786,2.0) (0.9686957182973392,-0.7330219075336785,2.0)
				(0.4686957182973392,-1.2330219075336784,2.0) (0.4686957182973392,-0.7330219075336785,2.0) (0.9686957182973392,-0.7330219075336785,2.0)
			};
		\addplot3 [patch,patch type=triangle, patch refines=0, shader=flat, opacity=0.15, color=acingreen] coordinates
			{
				(0.5586957182973392,-0.44302190753367837,0.7566626719988508) (0.47869571829733926,-0.5230219075336784,0.7566626719988508) (0.5586957182973393,-0.5230219075336784,0.7566626719988508)
				(0.5586957182973392,-0.44302190753367837,0.7566626719988508) (0.47869571829733926,-0.5230219075336784,0.7566626719988508) (0.47869571829733926,-0.44302190753367837,0.7566626719988508)
				(0.47869571829733926,-0.44302190753367837,1.006662671998851) (0.47869571829733926,-0.5230219075336784,0.7566626719988508) (0.47869571829733926,-0.44302190753367837,0.7566626719988508)
				(0.47869571829733926,-0.44302190753367837,1.006662671998851) (0.47869571829733926,-0.5230219075336784,1.006662671998851) (0.47869571829733926,-0.5230219075336784,0.7566626719988508)
				(0.47869571829733926,-0.44302190753367837,1.006662671998851) (0.5586957182973392,-0.44302190753367837,0.7566626719988508) (0.47869571829733926,-0.44302190753367837,0.7566626719988508)
				(0.47869571829733926,-0.44302190753367837,1.006662671998851) (0.5586957182973392,-0.44302190753367837,0.7566626719988508) (0.5586957182973392,-0.44302190753367837,1.006662671998851)
				(0.5586957182973393,-0.5230219075336784,1.006662671998851) (0.47869571829733926,-0.5230219075336784,0.7566626719988508) (0.5586957182973393,-0.5230219075336784,0.7566626719988508)
				(0.5586957182973393,-0.5230219075336784,1.006662671998851) (0.47869571829733926,-0.5230219075336784,1.006662671998851) (0.47869571829733926,-0.5230219075336784,0.7566626719988508)
				(0.5586957182973393,-0.5230219075336784,1.006662671998851) (0.5586957182973392,-0.44302190753367837,0.7566626719988508) (0.5586957182973393,-0.5230219075336784,0.7566626719988508)
				(0.5586957182973393,-0.5230219075336784,1.006662671998851) (0.5586957182973392,-0.44302190753367837,0.7566626719988508) (0.5586957182973392,-0.44302190753367837,1.006662671998851)
				(0.5586957182973393,-0.5230219075336784,1.006662671998851) (0.47869571829733926,-0.44302190753367837,1.006662671998851) (0.47869571829733926,-0.5230219075336784,1.006662671998851)
				(0.5586957182973393,-0.5230219075336784,1.006662671998851) (0.47869571829733926,-0.44302190753367837,1.006662671998851) (0.5586957182973392,-0.44302190753367837,1.006662671998851)
			};


		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates {(0, 0, 0)};
		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates{(2.32691068649292, -0.6337637901306152, 0.41110029220581057)};
		\draw (axis cs:2.32691068649292, -0.6337637901306152, 0.31110029220581057) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{h, 0}$};

		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates{(0.5186957182973392, -0.48302190753367835, 0.961662671998850)};
		\draw (axis cs:0.5186957182973392, -1.12302190753367835, 0.9616626719988509) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{h, ho}$};

		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates{(-0.9067300803868508, -0.5777403559832155, 0.8118041792813402)};
		\draw (axis cs:-0.9067300803868508, -0.5777403559832155, 0.8118041792813402) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{h, f}$};

		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates{(0.49353350694834774, -0.2566223602427127, 0.7606581156393782)};
		\draw (axis cs:0.49353350694834774, -0.2566223602427127, 0.6206581156393782) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{0}$};

		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates{(0.5761461703654832, -0.4627136540583015, 0.8297219928918769)};
		\draw (axis cs:0.4890795894423669, -0.5081318827242907, 0.8437911848078921) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{ho}$};

		\addplot3[
			only marks,
			mark=*,
			mark size=1pt,
		] coordinates{(-0.4464148000467676, -0.2192111234588623, 0.7037999563464113)};
		\draw (axis cs:-0.44650080267280783, -0.3075765280398828, 0.7231554130968114) node[
			scale=1.0,
			anchor=base west,
			text=black,
			rotate=0.0
		]{\bfseries $\vec{p}_\mathrm{f}$};

	\end{axis}
\end{tikzpicture}

